Role of hydrogen on the generation and decay of point defects in amorphous silica exposed to UV laser radiation

This experimental PhD work deals with the generation and transformation processes of point defects induced by UV laser irradiation on amorphous silicon dioxide (silica). The investigation relies on several spectroscopic techniques used to probe the microscopic damage induced by UV laser on the material. The most innovative approach, however, is the measurement in situ of the absorption signals related to laser-induced point defects. This technique yields new information on the kinetics of defect processes, inaccessible to previous works based only on stationary measurements of laser-induced damage. The main result is to show that a major damage mechanism of silica under 4.7eV laser radiation is the generation of E' centers (silicon dangling bond defects) by photolysis of pre-existing Si-H bonds. This process occurs by two-photon absorption of laser light, and the produced E' centers are unstable in a wide temperature range: in fact, rupture of Si-H produces hydrogen atoms H together with E'; hence, H atoms dimerize in H_2, which diffuses in the glass and reacts back with the E' centers causing their decay. The generation and decay kinetics of laser-induced E' centers are quantitatively modelled by considering the competition between the laser-induced breakage of Si-H and the concurrent reaction between E' and H_2. The latter reaction is studied in detail at several temperatures: some of its features are found to be affected by the disorder of the glass matrix; moreover, its kinetics is found to be activation-limited rather than diffusion-limited, contrary to what is usually found for the reactions of diffusing species with point defects.

==> Definizioni.tex <==
\newcommand{\sil}{$a-$SiO$_2$}
\makeatletter
\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\bibname}{\bibname}%
      \list{\@biblabel{\textbf{\@arabic\c@enumiv}}}
           {\setlength{\itemsep}{0.0pt}
           \settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}


\renewcommand\tableofcontents{%
    \if@twocolumn
      \@restonecoltrue\onecolumn
    \else
      \@restonecolfalse
    \fi
    \chapter*{\contentsname
        \@mkboth{%
           \contentsname}{\contentsname}}%
\addcontentsline{toc}{chapter}{Contents}
%\pdfbookmark[0]{Contents}{toc}
    \@starttoc{toc}%
    \if@restonecol\twocolumn\fi
    }
\makeatother


%\definecolor{postitA}{rgb}{1,1,0.8}

\definecolor{postitA}{rgb}{1,1,0.9}
\definecolor{postitB}{rgb}{1,1,0.7}
\definecolor{postitC}{rgb}{0.7,0.16,0.16}
\setlength{\fboxrule}{3pt} \setlength{\fboxsep}{8pt}

\makeatletter

\newdimen\shadowsizeB
\shadowsizeB 0pt \setlength{\fboxrule}{0pt}
\setlength{\fboxsep}{0pt}

\def\shadowboxF{\VerbBox\@shadowboxF}
\def\@shadowboxF#1{%
  \setbox\@fancybox\hbox{\fcolorbox{postitA}{postitA}{#1}}%
  \leavevmode\vbox{%
    \hbox{\lower\shadowsizeB\hbox{%
      \resizebox*{2cm}{\ht\@fancybox+\dp\@fancybox}{\begin{minipage}[c]{2cm}\fcolorbox{postitC}{postitC}{\textcolor{postitC}{a}}\end{minipage}}}\kern -\fboxrule\copy\@fancybox}%
      }}

 \makeatother

